Change Detection Methods for Remote Sensing in the Last Decade: A Comprehensive Review

Change detection is an essential and widely utilized task in remote sensing that aims to detect and analyze changes occurring in the same geographical area over time, which has broad applications in urban development, agricultural surveys, and land cover monitoring. Detecting changes in remote sensing images is a complex challenge due to various factors, including variations in image quality, noise, registration errors, illumination changes, complex landscapes, and spatial heterogeneity. In recent years, deep learning has emerged as a powerful tool for feature extraction and addressing these challenges. Its versatility has resulted in its widespread adoption for numerous image-processing tasks. This paper presents a comprehensive survey of significant advancements in change detection for remote sensing images over the past decade. We first introduce some preliminary knowledge for the change detection task, such as problem definition, datasets, evaluation metrics, and transformer basics, as well as provide a detailed taxonomy of existing algorithms from three different perspectives: algorithm granularity, supervision modes, and learning frameworks in the methodology section. This survey enables readers to gain systematic knowledge of change detection tasks from various angles. We then summarize the state-of-the-art performance on several dominant change detection datasets, providing insights into the strengths and limitations of existing algorithms. Based on our survey, some future research directions for change detection in remote sensing are well identified. This survey paper will shed some light on the community and inspire further research efforts in the change detection task.

==> Sec/backup/dataset.tex <==
 \par \noindent \textbf{1. SAR-based Change Detection Datasets} 
 \begin{itemize}
     \item \textbf{The Yellow River Dataset.} This dataset~\cite{9982693} consists of two SAR images of the Yellow River Estuary in China, each with dimensions of 7666 $\times$ 7692 pixels. These images were captured by the Radarsat-2 satellite in June 2008 and June 2009, respectively, which are commonly utilized for studying changes in this region, making it a valuable resource for various change detection methods applied to the SAR images.
     %\textbf{The Yellow River dataset} contains two 7666 $\times$ 7692 SAR images of the Yellow River Estuary in China. The dataset was taken by the Radarsat-2 satellite in June 2008 and June 2009 respectively. It can be used to study the changes in the region from 2008 to 2009 and is therefore widely used in many methods to study change detection of SAR images~\cite{DBLP:journals/tgrs/ZhangJLYSL22, 9982693}.
     \item \textbf{The Bern Dataset.} This dataset~\cite{9829884} comprises two SAR images, each with dimensions of 301 $\times$ 301 pixels, covering the city of Bern, Switzerland. The images were acquired by the European Remote Sensing Satellite-2 (ERS-2) in April and May of 1999. Notably, the May 1999 image captured the impact of flooding caused by the Aare River on the airport in Bern City.
     %\textbf{The Bern dataset} consists of two SAR images of 301 $\times$ 301 pixels covering Bern City taken by the ERS-2 satellite. The images were taken in April 1999 and May 1999, during which time Aare River flooded the airport at Bern City~\cite{9829884}.
     % The LEVIR-CD dataset~\cite{Chen2020},  The CDD dataset~\cite{DBLP:journals/corr/abs-2108-07955}, The WHU Building dataset~\cite{8444434} and The SECOND dataset~\cite{DBLP:journals/tgrs/YangXLDYPZ22}
 \end{itemize}
 \par \noindent \textbf{2. Multi-Spectral Change Detection Datasets}
 \begin{itemize}
     \item \textbf{The LEVIR-CD Dataset.} This dataset is a comprehensive remote sensing change detection resource, containing 637 pairs of very high-resolution (VHR, 0.5 m/pixel) Google Earth images, each measuring 1024 $\times$ 1024 pixels. The dataset, as described by Chen \textit{et al.}~\cite{Chen2020}, centers on detecting building changes in American cities between 2002 and 2018, with a particular focus on building growth and decline
 
     \item \textbf{The CDD Dataset.} The CDD dataset~\cite{DBLP:journals/corr/abs-2108-07955}, also referred to as the season-varying dataset, is a collection of VHR (i.e. 0.03-1 m/pixel) images comprising seven pairs of images with dimensions of 4725 $\times$ 2700 pixels and four pairs with dimensions of 1900 $\times$ 1000 pixels. The dataset, sourced from Google Earth, focuses on capturing seasonal variations in natural objects of varying sizes.
    
     \item \textbf{The WHU Building Dataset.} It~\cite{8444434} comprises three distinct datasets: an aerial imagery dataset, a satellite imagery dataset, and a building change detection dataset (BCDD). The aerial imagery dataset covers the city of Christchurch, New Zealand, and contains images with a ground resolution of 0.75m. The satellite imagery dataset consists of two subsets. The first subset encompasses cities from all over the world and was collected by a variety of satellites, including QuickBird, Worldview series, IKONOS, ZY-3, etc. The second subset comprises six neighboring satellite images, covering an area of 550 k\rm ${m}^{2}$ in East Asia. The BCDD is composed of a pair of images with a resolution of 15354 $\times$ 32507 pixels, capturing an area both before and after a 6.3-magnitude earthquake. This dataset is particularly useful for researchers interested in building damage detection and assessment after natural disasters, as well as for those interested in developing machine learning algorithms for automated building change detection.
    
    \item \textbf{The SECOND Dataset.} The second dataset~\cite{DBLP:journals/tgrs/YangXLDYPZ22}, as a semantic change detection dataset, is comprised of 4662 pairs of aerial images, obtained by several platforms and sensors. The dataset covers cities such as Hangzhou, Chengdu, and Shanghai, and each image pair has the same dimensions of 512 $\times$ 512 pixels, with a spatial resolution varying from 0.5 to 3 m/pixel. This dataset is particularly useful for researchers interested in studying man-made geographical and natural changes, covering six main categories. For the change category, the SECOND dataset focuses on 6 main land-cover classes, i.e., non-vegetated ground surface, trees, low vegetation, water, buildings, and playgrounds.

 \end{itemize}
  %\par \textbf{1) BANDON Dataset} The BANDON dataset is designed for building change detection using off-nadir aerial images. It consists of 2283 image pairs from urban and rural areas with corresponding change, BT-flows, segmentation, and ST-offsets labels (test sets don't have auxiliary annotations). BANDON provides novel data for the off-nadir building change detection task, and its detailed annotations support multi-task learning in aerial images.Paper: Pang \textit{et al.}2023 %(Building Change Detection with Off-nadir Aerial Images Dataset) 
%\par \textbf{2) MSBC Dataset} 2022.Multisource built-up change (MSBC) and multisource OSCD (MSOSCD) datasets The datasets are made to fill the gap of built-up CD datasets including multi-spectral, SAR, and VHR. MSBC is labeled based on GF-2 VHR images, and the MSOSCD is reformed from an existing dataset—Onera Satellite CD(OSCD) dataset. Paper: Li \textit{et al.}2022
%\par \textbf{3) CLCD dataset}
%The CLCD dataset consists of 600 pairs image of cropland change samples, with 320 pairs for training, 120 pairs for validation and 120 pairs for testing. The bi-temporal images in CLCD were collected by Gaofen-2 in Guangdong Province, China, in 2017 and 2019, respectively, with spatial resolution ranged from 0.5 to 2 m. Each group of samples is composed of two images of 512 × 512 and a corresponding binary label of cropland change. The main types of change annotated in CLCD include buildings, roads, lakes and bare soil lands, etc. Paper: Liu \textit{et al.}2022

%\par \textbf{4) HTCD dataset}
%The HTCD dataset, a new Satellite-UAV heterogeneous image data set, was built using the satellite images from Google Earth and UAV images from Open Aerial Map. The size of the satellite image is 11 K×15 K pixels. While the UAV image is consisted of 15 image blocks, in total 1.38 M×1.04 M pixels. The ground resolutions of them are 0.5971 m and 7.465 cm, respectively. Images and labels are all stored in GeoTiff format with location information, for the convenience of further analysis and research. Paper: Shao \textit{et al.}2021

%\par \textbf{Multi-modal Supervised Change Detection Data}
%Sentinel-1 SAR data were provided on the basis of OSCD dataset for multimodal supervised change detection (SAR-SAR CD or Optical-SAR multi-modal CD). Paper: Ebel \textit{et al.}2021

%\par \textbf{S2Looking}
%S2Looking, a building change detection dataset that contains large-scale side-looking satellite images captured at varying off-nadir angles. It consists of 5000 registered bitemporal image pairs (size of 1024*1024, 0.5 ~ 0.8 m/pixel) of rural areas throughout the world and more than 65,920 annotated change instances. It provides two label maps to separately indicate the newly built and demolished building regions for each sample in the dataset. Paper: Shen \textit{et al.}2021

%\par \textbf{SYSU-CD}
%The dataset contains 20000 pairs of 0.5-m aerial images of size 256×256 taken between the years 2007 and 2014 in Hong Kong.The main types of changes in the dataset include: (a) newly built urban buildings; (b) suburban dilation; (c) groundwork before construction; (d) change of vegetation; (e) road expansion; (f) sea construction. Paper: Shi \textit{et al.}2021

%\par \textbf{S2MTCP Dataset}
%The S2MTCP dataset contains N = 1520 image pairs, spread over all inhabited continents, with the highest concentration of image pairs in North-America, Europe, and Asia. Bands with a spatial resolution smaller than 10 m are resampled to 10 m and images are cropped to approximately 600x600 pixels. It was created for self-supervised training. Paper: Leenstra \textit{et al.}2021 % 2021.Sentinel-2 Multitemporal Cities Pairs (S2MTCP) dataset

%\par \textbf{DSIFN Dataset}
%The dataset is manually collected from Google Earth. It consists of six large bi-temporal high resolution images covering six cities (i.e., Beijing, Chengdu, Shenzhen, Chongqing, Wuhan, Xian) in China. The five large image-pairs (i.e., Beijing, Chengdu, Shenzhen, Chongqing, Wuhan) are clipped into 394 subimage pairs with sizes of 512×512. After data augmentation, a collection of 3940 bi-temporal image pairs is acquired. Xian image pair is clipped into 48 image pairs for model testing. There are 3600 image pairs in the training dataset, 340 image paris in the validation dataset, and 48 image pairs in the test dataset. Paper: Zhang \textit{et al.}2020

%\par \textbf{SECOND Dataset}
%SECOND, a well-annotated semantic change detection dataset, which collects 4662 pairs of aerial images from several platforms and sensors. These pairs of images are distributed over the cities such as Hangzhou, Chengdu, and Shanghai. Each image has size 512 x 512 and is annotated at the pixel level. SECOND focus on 6 main land-cover classes, i.e. , non-vegetated ground surface, tree, low vegetation, water, buildings, and playgrounds, that are frequently involved in natural and man-made geographical changes. Paper: Yang \textit{et al.}2020. % 2020.SEmantic Change detectiON Dataset (SECOND)

%\par \textbf{Google Dataset}
%The images were acquired during the periods between 2006 and 2019, covering the suburb areas of Guangzhou City, China. To facilitate image pair generation, Google Earth service through the BIGEMAP software was adopted to collect 19 season-varying VHR images pairs with three bands of red, green, and blue, a spatial resolution of 0.55 m, and the size ranging from 1006×1168 pixels to 4936×5224 pixels. The annotation is focused on buildings. Paper: Peng \textit{et al.}2020

%\par \textbf{LEVIR-CD}
%LEVIR-CD consists of 637 very high-resolution (VHR, 0.5m/pixel) Google Earth image patch pairs with a size of 1024 × 1024 pixels. These bitemporal images with time span of 5 to 14 years have significant land-use changes, especially the construction growth. LEVIR-CD covers various types of buildings, such as villa residences, tall apartments, small garages and large warehouses. The fully annotated LEVIR-CD contains a total of 31,333 individual change building instances. LEVIR-CD+ can be found in this page. Paper: Chen \textit{et al.}2020. % 2020.LEVIR building Change Detection (LEVIR-CD) Dataset

%\par \textbf{HRSCD}
%This dataset contains 291 coregistered image pairs of RGB aerial images from IGS's BD ORTHO database. Pixel-level change and land cover annotations are provided, generated by rasterizing Urban Atlas 2006, Urban Atlas 2012, and Urban Atlas Change 2006-2012 maps. Paper: Daudt \textit{et al.}2019 % 2019.High Resolution Semantic Change Detection (HRSCD) Dataset

%\par \textbf{MtS-WH}
%The dataset is mainly used for theoretical research and verification of scene change detection methods. It consists of two large-size VHR images, which have a size of 7200x6000 and are respectively acquired by IKONOS sensors in Feb 2002 and Jun 2009. The images cover the Hanyang District, Wuhan City, China and contain 4 spectral bands (Blue, Green, Red, and Near-Infrared). The spatial resolution of the images is 1m after fusion of the pan and multi-spectral images by the Gram–Schmidt algorithm. For a discussion of this dataset, please refer to \#3. Paper: Wu \textit{et al.}2017 % 2019.Wuhan multi-temperature scene (MtS-WH) Dataset

%\par \textbf{WHU}
%The dataset contains two aerial images (0.2m/pixel, 15354×32507) and provides a change vector, a change raster map, and two corresponding building vectors of these two aerial images. Paper: Ji \textit{et al.}2018

%\par \textbf{Synthetic images and real season-varying remote sensing images}
%This dataset has three types: synthetic images without objects relative shift, synthetic images with small relative shift of objects, real season-varying remote sensing images (obtained by Google Earth). The real season-varying remote sensing images have 16000 image sets with image size 256x256 pixels (10000 train sets and 3000 test and validation sets) and a spatial resolution of 3 to 100 cm/px. For a discussion of this dataset, please refer to \#5. Paper: Lebedev \textit{et al.}2018

%\par \textbf{Onera Satellite Change Detection Dataset}
%This dataset addresses the issue of detecting changes between satellite images from different dates. It comprises 24 pairs of multi-spectral images taken from the Sentinel-2 satellites between 2015 and 2018. Locations are picked all over the world, in Brazil, USA, Europe, Middle-East and Asia. For each location, registered pairs of 13-band multi-spectral satellite images obtained by the Sentinel-2 satellites are provided. Images vary in spatial resolution between 10m, 20m, and 60m. Paper: Daudt \textit{et al.}2018

%\par \textbf{AICD} 
%This dataset contains synthetic aerial images with artificial changes generated with a rendering engine. It contains 1000 pairs of 800x600 images, each pair consisting of one reference image and one test image, and the 1000 corresponding 800x600 ground truth masks. Paper: Bourdis \textit{et al.}2011 % 2011.The Aerial Imagery Change Detection (AICD) dataset

%\par \textbf{SZTAKI AirChange Benchmark set}
%This dataset contains 13 aerial image pairs of size 952x640 and resolution 1.5m/pixel and binary change masks (drawn by hand). Each record contains a pair of preliminary registered input images and a mask of the 'relevant' changes. The input images are taken with 5, 7 resp. 23 years of time differences. During the generation of the change mask, we have considered the following differences as relevant changes: (a) new built-up regions (b) building operations (c) planting of large group of trees (d) fresh plow-land (e) groundwork before building over. Note that the ground truth does NOT contain change classification, only binary change-no change decision for each pixel. Paper: Benedek \textit{et al.}2008

\par \noindent \textbf{3. Hyper-Spectral Change Detection Datasets}
\begin{itemize}
    \item \textbf{The River Dataset.} It~\cite{Wang2019GETNETAG} comprises two Hyperspectral Images (HSI) \xt{hyperspectral images (HSI), please check the entire draft. } sized 463 $\times$ 241 pixels. The images were captured on May 3 and December 21, 2013, respectively, and primarily cover a river in Jiangsu Province. The dataset is centered on the detection of the absence of substances in rivers and comprises 198 bands after the elimination of noisy bands.
    %\textbf{The River dataset} consists of two HSIs with a size of 463 $\times$ 241 pixels.The images which mainly cover a river in Jiangsu Province were acquired on May 3, 2013 and December 21, 2013, respectively. The dataset focuses on the disappearance of substances in rivers and includes 198 bands after noisy band removal~\cite{Wang2019GETNETAG}.
    \item \textbf{The Hermiston Dataset.} The Hermiston dataset~\cite{DBLP:journals/tgrs/WangWWWB22} encompassing an agricultural area in Hermiston city was obtained by Hyperion sensor. The dataset contains a pair of HSIs collected on May 1, 2004, and May 8, 2007, respectively. The images have a resolution of 307 $\times$ 241 pixels and comprise a selection of 154 bands from a total of 242 spectral bands. The main change type on this dataset is the management of irrigation areas.
    \end{itemize}
%\par \textbf{Hyperspectral Change Detection Dataset} This dataset can be used to perform change detection techniques in multi-temporal hyperspectral images. It includes two different hyperspectral scenes from the AVIRIS sensor: The Santa Barbara scene, taken on the years 2013 and 2014 with the AVIRIS sensor over the Santa Barbara region (California) whose spatial dimensions are 984 x 740 pixels and includes 224 spectral bands. The Bay Area scene, taken on the years 2013 and 2015 with the AVIRIS sensor surrounding the city of Patterson (California) whose spatial dimensions are 600 x 500 pixels and includes 224 spectral bands. It also includes a hyperspectral scene from the HYPERION sensor: The Hermiston city scene, taken on the years 2004 and 2007 with the HYPERION sensor over the Hermiston City area (Oregon) whose spatial dimensions are 390 x 200 pixels and includes 242 spectral bands. 5 types of changes related to crop transitions are identified in this scene. Paper: López-Fandiño \textit{et al.}2018

%\par \textbf{GETNET} This dataset has two hyperspectral images, which were acquired on May 3, 2013, and December 31, 2013, respectively in Jiangsu province, China. It has a size of 463×241 pixels, with 198 bands available after noisy band removal. In the ground-truth map, white pixels represent changed portions and black pixels mean unchanged parts. Paper: Wang \textit{et al.}2018

\par \noindent \textbf{4. Heterogeneous Change Detection Datasets}
\begin{itemize}
    \item \textbf{The California Dataset.} This dataset~\cite{DBLP:journals/tnn/YangJLHYJ22} contains one multi-spectral image and two SAR images. The multi-spectral image was collected on January 5, 2017 by Landsat-8. Most bands in it have a resolution of 30m. While the SAR images were captured on February 18, 2017 by Sentinel-1A. The dataset covers the same region in Sacramento County, Yuba County, and Sutter County, California, where flood has caused the changes.
\end{itemize}

\par \noindent \textbf{5. 3D Point Cloud Change Detection Datasets}
\begin{itemize}
    \item \textbf{The 3DCD Dataset.} This dataset~\cite{isprs-archives-XLIII-B3-2022-1349-2022} comprises a total of 472 image pairs, each consisting of optical orthophotos cropped to the same size, along with the corresponding 2D change detection maps in raster format. The images were obtained by two aerial surveys in 2010 and 2017 separately. 472 pairs of Digital Surface Models (DSMs) produced from the rasterization of point clouds and the corresponding 3D change detection maps are also included in the dataset. The 2D change detection maps have a resolution of 0.5m with a size of 400 $\times$ 400 pixels. While the 3D change detection maps have a resolution of 1m with a size of 200 $\times$ 200 pixels. The dataset focuses on the urban area of Valladolid, Spain.
\end{itemize}
%\par \textbf{Change3D}

%\par \textbf{}~\cite{MARSOCCI2023325} ~\cite{isprs-archives-XLIII-B3-2022-1349-2022}

\subsection{Evaluation Metrics} %\gl{Yunmeng try to write this subsection}
%\par It is a widely recognized fact that evaluation metrics play a critical role in assessing the performance of a change detection model. To this end, we provide a concise introduction and analysis of certain prevalent evaluation metrics. The following are the measurements that are widely utilized:
%\begin{equation}
%    Precision = \frac{TP}{TP + FP},
%\end{equation}
%\begin{equation}
%    Recall = \frac{TP}{TP + FN},
%\end{equation}
%\begin{equation}
%    IoU = \frac{TP}{TP + FN + FP},
%\end{equation}
%\begin{equation}
%    OA = \frac{TP + TN}{TP + FP + TN + FN},
%\end{equation}
%\begin{equation}
%     F_{1} = \frac{2TP}{2TP + FP + FN},
%\end{equation}
%\begin{equation}
 %   RMSE = \sqrt{\frac{1}{n}\sum_{i=1}^{n}(\widehat{\Delta{H_{i}}}-{\Delta{H_{i}}})^{2}} ,
%\end{equation}
%\begin{equation}
 %   cRMSE = \sqrt{\frac{1}{n_{c}}\sum_{i=1}^{n_{c}}(\widehat{\Delta{H_{i}}}^{C}-{\Delta{H_{i}^{C}}})^{2}} ,
%\end{equation}
%where TP (True Positive) and TN (True Negative) represent the number of changed and unchanged pixels, respectively, that have been correctly identified by the algorithm. FP (False Positive) and FN (False Negative) denote the number of pixels that have been incorrectly classified as changed or unchanged, respectively. A higher precision value indicates that the algorithm is more precise in correctly identifying changed pixels, whereas a higher recall value indicates that the algorithm is able to detect a higher proportion of actual changed pixels among all the changed pixels in the ground truth data. A higher precision indicates that the model is more accurate in determining whether the pixel has changed, while a higher recall indicates that the model is looking for more changed pixels. The IoU (Intersection over Union) metric is defined as the ratio of intersection and concatenation of the predicted map and ground truth. The OA (Overall Accuracy) metric indicates the accuracy of the prediction results. The $F_{1}$ (F1-score) is a harmonic average of precision and recall. In addition, there are some other metrics designed for special applications. The Kappa coefficient~\cite{Rosenfield1986ACO} is used to measure classification accuracy and is calculated based on the confusion matrix. The RMSE (Root Mean Squared Error) and cRMSE (Changed Root Mean Squared Error)~\cite{MARSOCCI2023325} are commonly used to evaluate the change detection performance of 3D point cloud models. In particular, cRMSE is a RMSE considering only the errors about ground truth pixels that are influenced by altitude. While in the semantic change detection (SCD) task, 3 other metrics are commonly adopted to evaluate the accuracy, including mean Intersection over Union (mIoU) , Separated Kappa (Sek) coefficient and SCD-targeted F1 Score ($F_{scd}$)~\cite{Ding2022JointSM}. More detailed information about the 3 evaluation metrics can be found in~\cite{DBLP:journals/tgrs/DingGLMZB22}.

==> Sec/others.tex <==

 \begin{table*}[h]
  \centering
  \caption{Taxonomy based on Supervision Modes. \gl{put it in the appendix later}}
  \begin{tabular}{c|c|c|c}
    \hline\hline
    \rowcolor{gray!80!}  & \multicolumn{3}{c} {\textbf{Supervision Modes}} \\
    \hline
    \rowcolor{gray!30!}  & \textbf{Unsupervised} & \textbf{Semi-supervised} & \textbf{Supervised} \\
    \hline 
    \textbf{SAR based} & \makecell[l]{\cite{DBLP:journals/tgrs/ZhangJLYSL22} \cite{DBLP:journals/lgrs/WangZJL22} \cite{DBLP:journals/staeors/LopezS22} \cite{DBLP:journals/lgrs/AtaseverG22} \cite{9810349} \cite{DBLP:journals/staeors/PengCYZD22} \cite{DBLP:journals/tgrs/ZhuangHDZWY22} \cite{DBLP:journals/tgrs/AmitranoGI21} \\ \cite{DBLP:journals/staeors/LiXXWX22} \cite{DBLP:journals/lgrs/FangX22} \cite{DBLP:journals/lgrs/WangZJ22} \cite{DBLP:journals/tgrs/ZhangACC15} \cite{DBLP:journals/tgrs/BouhlelM20} \cite{DBLP:journals/tgrs/PirroneBB20} \cite{DBLP:journals/access/LiuJYK19} \cite{DBLP:journals/tgrs/WestR19} \\ \cite{DBLP:journals/lgrs/LiCLE15} \cite{DBLP:journals/staeors/LuLCZXK15} \cite{DBLP:journals/lgrs/WangDD16} \cite{DBLP:journals/lgrs/SumaiyaK16} \cite{DBLP:journals/tgrs/AkbariADEMS16} \cite{DBLP:journals/lgrs/Jia0ZWZ16} \cite{DBLP:journals/tgrs/YangYYSX16} \cite{DBLP:journals/staeors/WangJY16} \\ \cite{DBLP:journals/lgrs/RathaDCB17} \cite{DBLP:journals/tgrs/WangZDZH22} \cite{DBLP:journals/tgrs/ZhuangFDZWW22} \cite{DBLP:journals/lgrs/YuY22} \cite{DBLP:journals/lgrs/LiuWHLJ21} \cite{9894362} \cite{DBLP:journals/lgrs/LiuCL22} \\ \cite{DBLP:journals/tgrs/VuGPDH19} \cite{DBLP:journals/tgrs/LiPCJZS19} \cite{9982693}} & \makecell[l]{\cite{DBLP:journals/lgrs/WangSG22} \cite{DBLP:journals/staeors/WangWCL21} \cite{DBLP:journals/lgrs/WangWWCJ22}} & \makecell[l]{\cite{DBLP:journals/staeors/SahaSEZ22} \cite{DBLP:journals/lgrs/ChenZWY23} \cite{DBLP:journals/lgrs/VinholiSMP22}  \cite{DBLP:journals/lgrs/ShiLL21} \cite{DBLP:journals/lgrs/ZhangSYW22} \cite{DBLP:journals/lgrs/LiLZWSA19} \\ \cite{DBLP:journals/lgrs/GaoWGDW19} \cite{DBLP:journals/tgrs/GengMZW19} \cite{DBLP:journals/lgrs/LiLZSA015} \cite{DBLP:journals/lgrs/GaoDLX16} \cite{DBLP:journals/tnn/GongZLMJ16} \cite{DBLP:journals/lgrs/CamposPVM22} \cite{DBLP:journals/staeors/GaoGDW19} \\ \cite{DBLP:journals/lgrs/QuGDDL22} \cite{DBLP:journals/lgrs/MengGDDL22} \cite{DBLP:journals/tgrs/VinholiPSMP22} \cite{DBLP:journals/staeors/WangGDZD22}} \\
    \hline
    \textbf{Multi-spectral based} & \makecell[l]{\cite{DBLP:journals/tip/TouatiMD20} \cite{DBLP:journals/staeors/KalinichevaIST20} \cite{DBLP:journals/lgrs/WangCBLC15} \cite{DBLP:journals/lgrs/HaoZJS20} \cite{DBLP:journals/tgrs/ZhanGJZ20} \cite{DBLP:journals/tgrs/WangAS15a} \cite{DBLP:journals/lgrs/DingHXZP15} \\ \cite{DBLP:journals/tip/ZanettiBB15}  \cite{DBLP:journals/lgrs/AleksandrowiczW16} \cite{DBLP:journals/lgrs/ZhangGZSS16} \cite{DBLP:journals/tgrs/HedjamKMNC16} \cite{DBLP:journals/tgrs/DuRWZ19} \cite{DBLP:journals/tgrs/Padron-HidalgoL19} \cite{DBLP:journals/tgrs/LvLZBLZ19} \\ \cite{DBLP:journals/tgrs/LiLFD16} \cite{DBLP:journals/staeors/ZhouCLS16} \cite{DBLP:journals/tip/KrylovMSZ16} \cite{DBLP:journals/lgrs/WuD17} \cite{DBLP:journals/tgrs/GongZZM17} \cite{DBLP:journals/staeors/0012LNZL17} \cite{DBLP:journals/lgrs/HouWL17} \\ \cite{DBLP:journals/lgrs/LiSZH17} \cite{DBLP:journals/lgrs/WuLFMS18} \cite{DBLP:journals/lgrs/GuptaPA18} \cite{DBLP:journals/staeors/ZhangLC18} \cite{DBLP:journals/lgrs/ZhangPH18} \cite{DBLP:journals/tgrs/ZanettiB18} \cite{DBLP:journals/tgrs/LiuGT19} \\ \cite{DBLP:journals/staeors/GongYZNL19} \cite{DBLP:journals/staeors/FanLH19} \cite{DBLP:journals/tgrs/YangLWYE19} \cite{DBLP:journals/lgrs/CorreaBB19} \cite{DBLP:journals/tgrs/LvLB20} \cite{DBLP:journals/lgrs/ZhangLZSZ22} \cite{DBLP:journals/tgrs/BergamascoSBB22} \\ \cite{DBLP:journals/lgrs/ShiZTLL22} \cite{DBLP:conf/cvpr/NohJSPC22} \cite{DBLP:journals/staeors/XiaoWCSQL23} \cite{DBLP:journals/tgrs/LiuYZDL22} \cite{DBLP:journals/tgrs/Padron-HidalgoL22} \cite{DBLP:journals/tcyb/WuCDZ22} \cite{DBLP:journals/lgrs/ShaoYLDR22} \\  \cite{DBLP:journals/lgrs/LvWLKB22} \cite{DBLP:journals/lgrs/FangDWLT22} \cite{DBLP:journals/lgrs/GuoZZZ22} \cite{DBLP:journals/lgrs/Radoi22} \cite{DBLP:journals/tgrs/MouHSBBZ22} \cite{DBLP:journals/tgrs/ChenB22b} \cite{DBLP:journals/tgrs/TangZMLZZJ22} \\ \cite{DBLP:journals/tgrs/RenWGZC21} \cite{DBLP:journals/staeors/XueLJWCN21} \cite{DBLP:journals/staeors/ZhouSCZSQ21} \cite{DBLP:journals/staeors/TangWZ21} \cite{DBLP:journals/tgrs/GuoZ021} \cite{DBLP:journals/lgrs/SahaCBB21} \cite{DBLP:journals/tgrs/NegriFCADSA21} \cite{9828490}} & \makecell[l]{\cite{DBLP:journals/lgrs/JiangGZF20} \cite{DBLP:journals/tgrs/ZhangLL18} \cite{DBLP:journals/staeors/HedjamAM20} \\ \cite{DBLP:journals/tgrs/ShiWQLJ22} \cite{DBLP:conf/igarss/HafnerBN22} \cite{DBLP:journals/tgrs/ChenLCS22} \\ \cite{9978928} \cite{DBLP:journals/lgrs/SahaMZBB21} \cite{DBLP:journals/tgrs/PengBZGDH21} \\ \cite{DBLP:journals/remotesensing/ZhangSLP19} \cite{DBLP:journals/sensors/HouWL16} \cite{DBLP:conf/igarss/AlvarezRD20}} & \makecell[l]{\cite{DBLP:journals/lgrs/ZhongLZZ15} \cite{DBLP:journals/lgrs/ZhangYGYSYZ22} \cite{DBLP:journals/lgrs/LiHLS22} \cite{DBLP:journals/lgrs/XiangTLY22} \cite{DBLP:journals/tgrs/ShiLLLWZ22} \cite{DBLP:journals/lgrs/PeiZ22} \cite{DBLP:journals/lgrs/LinLFG20} \\  \cite{DBLP:journals/tgrs/HeZZ20} \cite{DBLP:journals/tgrs/HouLWW20} \cite{DBLP:journals/tgrs/ZhaoMCBE20} \cite{DBLP:journals/lgrs/MesquitaSMCN20} \cite{DBLP:journals/tgrs/ZhangS20} \cite{DBLP:journals/tgrs/VongsyEM15} \cite{DBLP:journals/tgrs/MouBZ19} \\ \cite{DBLP:journals/staeors/TanJPWXD16} \cite{DBLP:journals/lgrs/ZhanFYSWQ17} \cite{DBLP:journals/tgrs/KhanHPB17} \cite{DBLP:journals/staeors/KernerWBGBA19} \cite{DBLP:journals/lgrs/ZhangXCYS19} \cite{DBLP:journals/tgrs/YangJLHY19} \cite{DBLP:journals/lgrs/KhuranaS20} \\ \cite{DBLP:journals/staeors/WangDCLZL20} \cite{DBLP:journals/tgrs/ChenWDZW20} \cite{DBLP:journals/staeors/LiuJZZ20} \cite{DBLP:journals/lgrs/BaoFFH20} \cite{DBLP:journals/corr/abs-2212-01287} \cite{DBLP:journals/corr/abs-2206-11892} \cite{DBLP:journals/corr/abs-2108-07955} \\ \cite{DBLP:journals/staeors/ZhaoZGLYXL22} \cite{DBLP:journals/tgrs/LvWCBLS22} \cite{9721892} \cite{DBLP:journals/tcsv/ZhouWZYCM22} \cite{DBLP:journals/corr/abs-2212-04869} \cite{DBLP:journals/corr/abs-2212-05245} \cite{DBLP:journals/corr/abs-2207-09240} \\ \cite{DBLP:journals/corr/abs-2211-11478} \cite{DBLP:journals/staeors/YuanWC22} \cite{DBLP:journals/staeors/SongXWLQC23} \cite{10023508} \cite{DBLP:journals/tgrs/LiuSMHLZ22} \cite{DBLP:journals/tgrs/LiTLZDWZ23} \cite{DBLP:journals/tgrs/LiZDD22} \\ \cite{DBLP:journals/tgrs/HuangSWY22} \cite{DBLP:journals/staeors/SongHL22} \cite{9721897} \cite{DBLP:journals/tgrs/ChengWH22} \cite{DBLP:journals/tgrs/FengXJLZ22} \cite{DBLP:journals/tgrs/ZhouFHL22} \cite{DBLP:journals/corr/abs-2202-09745} \\ \cite{DBLP:journals/lgrs/LiYZM22} \cite{DBLP:journals/tgrs/LiTWZ22} \cite{DBLP:journals/tgrs/ChenQS22} \cite{DBLP:journals/staeors/ShiLZWHZSLLZ22} \cite{DBLP:journals/lgrs/SunZHWX22} \cite{DBLP:journals/staeors/HeCLC22} \cite{DBLP:journals/lgrs/JianCC22} \\ \cite{DBLP:journals/tgrs/LeiWNWX0N22} \cite{DBLP:journals/staeors/ChouhanSC22} \cite{DBLP:journals/lgrs/JiangXWT22} \cite{DBLP:journals/lgrs/RazaHF22} \cite{DBLP:journals/staeors/DengCYYMCZ22} \cite{DBLP:journals/tgrs/BaiFLL22} \cite{DBLP:journals/lgrs/XuOLWT22} \\ \cite{DBLP:journals/tgrs/YangXLDYPZ22} \cite{DBLP:journals/tgrs/YuanMXZ22} \cite{DBLP:journals/lgrs/SunMWL22} \cite{DBLP:journals/lgrs/HanLZ22} \cite{DBLP:journals/lgrs/SongZLSP22} \cite{DBLP:journals/lgrs/DuZDLCZC22} \cite{DBLP:journals/staeors/ChenLYZDP22} \\  \cite{DBLP:journals/tgrs/ZhangTXYLYXJZ22} \cite{DBLP:journals/tgrs/XiaTZL22} \cite{DBLP:journals/corr/abs-2208-08292} \cite{DBLP:journals/corr/abs-2302-10420} \cite{DBLP:journals/corr/abs-2302-05109} \cite{DBLP:journals/lgrs/LiuPZZY21} \cite{DBLP:journals/staeors/ChenYPCHZLL21} \\ \cite{DBLP:journals/tnn/ZhangLYZ23} \cite{DBLP:journals/staeors/LuoLWHWJX21} \cite{DBLP:journals/tgrs/YangJHLY21} \cite{DBLP:journals/staeors/LiuCDL22} \cite{DBLP:journals/tgrs/DingGLMZB22} \cite{DBLP:journals/tgrs/LiuGLZZJZ22} \\ \cite{DBLP:journals/tgrs/GuoZZZZ22} \cite{DBLP:journals/staeors/SongDL22} \cite{DBLP:journals/lgrs/ZhaoCGC22} \cite{doi:10.1080/01431161.2021.1941390}} \\
    \hline
    \textbf{Hyper-spectral based} & \makecell[l]{\cite{DBLP:journals/staeors/HuWZD21} \cite{DBLP:journals/tgrs/MeolaEMA12} \cite{DBLP:journals/tgrs/EismannMH08} \cite{8898697} \cite{DBLP:journals/ijon/WuZD15} \cite{DBLP:journals/tgrs/MarinelliBB19} \cite{DBLP:journals/lgrs/ErturkP15} \\ \cite{DBLP:journals/tgrs/LiuBBD15} \cite{DBLP:journals/staeors/ErturkIP16} \cite{DBLP:journals/staeors/JafarzadehH19} \cite{DBLP:journals/staeors/TongPLLLXX20} \cite{DBLP:journals/staeors/LiGDLHWFHTLM21} \cite{DBLP:journals/staeors/LiuHNG22} \cite{DBLP:journals/tip/HuWDZ23} \\ \cite{DBLP:journals/tgrs/ChangKG22} \cite{DBLP:journals/lgrs/DingLZ22} \cite{DBLP:journals/tgrs/WangWWB22} \cite{DBLP:journals/tgrs/GongJQLZLZZ22} \cite{DBLP:journals/tgrs/QuHDLX22} \cite{DBLP:journals/tgrs/HuWZ22} \cite{DBLP:journals/tgrs/LuoZLGGR23} \\ \cite{DBLP:journals/staeors/GeTBZXS22} \cite{DBLP:journals/tgrs/WangWWWB22} \cite{DBLP:journals/staeors/ZhanSSJWYW21} \cite{DBLP:journals/lgrs/ZhaoCF22} \cite{DBLP:journals/tgrs/ShiZZZX22} \cite{DBLP:conf/igarss/Hu0022}} & \makecell[l] {\cite{DBLP:journals/staeors/LiuHNG22} \cite{DBLP:journals/ijon/YuanLL15} \cite{Wang2019GETNETAG} \\ \cite{DBLP:journals/jvcir/HuangYF19}} & \makecell[l]{ \cite{DBLP:journals/tip/HuWDZ23} \cite{DBLP:journals/tgrs/ChangKG22} \cite{DBLP:journals/lgrs/DingLZ22} \cite{DBLP:journals/tgrs/WangWWB22} \cite{DBLP:journals/tgrs/GongJQLZLZZ22} \cite{DBLP:journals/tgrs/QuHDLX22} \cite{DBLP:journals/tgrs/HuWZ22} \\ \cite{DBLP:journals/tgrs/LuoZLGGR23} \cite{DBLP:journals/staeors/GeTBZXS22} \cite{DBLP:journals/tgrs/WangWWWB22} \cite{DBLP:journals/staeors/ZhanSSJWYW21} \cite{DBLP:journals/lgrs/ZhaoCF22} \cite{DBLP:journals/tgrs/ShiZZZX22} \cite{DBLP:conf/igarss/Hu0022}} \\
    \hline
    \textbf{Heterogeneous based} & \makecell[l]{\cite{DBLP:journals/staeors/ZhouLSWL21} \cite{DBLP:conf/igarss/TomenottiLHMA20} \cite{DBLP:conf/igarss/HanTC22} \cite{DBLP:journals/lgrs/JiaZLZW22} \cite{DBLP:journals/tgrs/ZhaoWGL17} \cite{DBLP:journals/tnn/WuLYQMG22} \cite{DBLP:journals/tgrs/LuppinoKBMSJA22} \\ \cite{DBLP:journals/tip/SunLGK21} \cite{DBLP:journals/lgrs/ZhanGJL18} \cite{DBLP:journals/staeors/ChenHL22} \cite{DBLP:journals/staeors/LiGZW21} \cite{DBLP:journals/tgrs/SunLLTK21} \cite{DBLP:journals/tgrs/SunLGLK22} \cite{DBLP:journals/tgrs/LiuZPN22} \\ \cite{DBLP:journals/tgrs/SunLLTK22} \cite{DBLP:journals/tip/PrendesC0GT15} \cite{DBLP:journals/staeors/TouatiMD19} \cite{DBLP:journals/staeors/TouatiMD20a} \cite{DBLP:journals/lgrs/LeiSK22} \cite{DBLP:journals/tgrs/SahaEZ22} \cite{DBLP:journals/tgrs/HuLX22}} & \cite{DBLP:journals/tgrs/JiangLZH22} \cite{DBLP:journals/aeog/WuLQNZFS21} & \makecell[l]{\cite{DBLP:conf/igarss/MoserALS20} \cite{DBLP:conf/icpr/Yang0CF18} \cite{DBLP:journals/staeors/JiangLLZH20} \cite{DBLP:journals/tip/LiuLMHP18} \cite{DBLP:journals/tgrs/WangL22b} \cite{DBLP:journals/tnn/LiuGQZ18} \cite{DBLP:journals/lgrs/NiuGZY19} \\ \cite{DBLP:journals/tgrs/WanXY19} \cite{DBLP:journals/lgrs/LvHGBZS22} \cite{DBLP:journals/tnn/YangJLHYJ22}} \\
    \hline
    \textbf{3D point cloud based} & \makecell[l] {\cite{DBLP:journals/staeors/XiaoXEV16} \cite{DBLP:journals/tgrs/MarinelliPB18} \cite{DBLP:conf/igarss/MarinelliCBB18} \cite{doi:10.1080/17538947.2019.1585975} \cite{8272508} \cite{isprs-annals-IV-2-W7-9-2019} \cite{isprs-annals-V-2-2020-687-2020} \cite{isprs-annals-IV-2-W5-357-2019}} &  & \cite{MARSOCCI2023325, DEGELIS2023274} \\
    \hline\hline
  \end{tabular}
  \label{tab:data_supervision_backup}
\end{table*}



  \begin{table*}[h]
  \centering
  \caption{Taxonomy based on Learning Frameworks. \gl{put it in the appendix later}}
  \begin{tabular}{c|c|c|c}
    \hline\hline
    \rowcolor{gray!80!}  & \multicolumn{3}{c} {\textbf{Learning Frameworks}} \\
    \hline
    \rowcolor{gray!30!}  & \textbf{Traditional} & \textbf{CNN} & \textbf{Attention or Transformer} \\
    \hline
    \textbf{SAR based} & \makecell[l]{\cite{DBLP:journals/staeors/SahaSEZ22} \cite{DBLP:journals/lgrs/WangZJL22} \cite{DBLP:journals/tgrs/WangZDZH22} \cite{DBLP:journals/tgrs/ZhuangFDZWW22} \cite{DBLP:journals/lgrs/ChenZWY23} \cite{DBLP:journals/lgrs/YuY22} \\ \cite{DBLP:journals/tgrs/ZhangJLYSL22} \cite{DBLP:journals/lgrs/LiuCL22} \cite{DBLP:journals/staeors/PengCYZD22} \cite{DBLP:journals/tgrs/ZhuangHDZWY22} \cite{DBLP:journals/staeors/LopezS22} \cite{DBLP:journals/lgrs/AtaseverG22} \\ \cite{9810349} \cite{DBLP:journals/tgrs/AmitranoGI21}  \cite{DBLP:journals/staeors/LiXXWX22} \cite{DBLP:journals/lgrs/FangX22} \cite{DBLP:journals/lgrs/WangZJ22} \cite{DBLP:journals/tgrs/ZhangACC15} \\ \cite{DBLP:journals/tgrs/BouhlelM20} \cite{DBLP:journals/tgrs/PirroneBB20} \cite{DBLP:journals/access/LiuJYK19} \cite{DBLP:journals/tgrs/WestR19} \cite{DBLP:journals/lgrs/LiCLE15} \cite{DBLP:journals/staeors/LuLCZXK15} \\ \cite{DBLP:journals/staeors/NielsenCS15} \cite{DBLP:journals/lgrs/LiLZSA015} \cite{DBLP:journals/lgrs/WangDD16} \cite{DBLP:journals/lgrs/SumaiyaK16} \cite{DBLP:journals/tgrs/CarotenutoMCSA16} \cite{DBLP:journals/tgrs/AkbariADEMS16} \\ \cite{DBLP:journals/lgrs/Jia0ZWZ16} \cite{DBLP:journals/tgrs/YangYYSX16} \cite{DBLP:journals/staeors/WangJY16} \cite{DBLP:journals/lgrs/RathaDCB17} \cite{DBLP:journals/tgrs/McGuinnessB17} \cite{DBLP:journals/tgrs/VuPMDH17} \\ \cite{DBLP:journals/staeors/Ghanbari018} \cite{DBLP:journals/tgrs/LiZSSPCKL18} \cite{DBLP:journals/staeors/ZhangW0L018} \cite{DBLP:journals/lgrs/YangLYFSE19} \cite{DBLP:journals/tgrs/DominguezMMSSH19} \cite{DBLP:journals/tgrs/VuGPDH19}} & \makecell[l]{ \cite{9982693, DBLP:journals/lgrs/VinholiSMP22, DBLP:journals/lgrs/WangWWCJ22, DBLP:journals/lgrs/ShiLL21, DBLP:journals/lgrs/LiuWHLJ21, 9894362, DBLP:journals/lgrs/WangSG22} \\ \cite{DBLP:journals/lgrs/ZhangSYW22, DBLP:journals/lgrs/CamposPVM22, DBLP:journals/staeors/WangWCL21, DBLP:journals/lgrs/LiLZWSA19, DBLP:journals/lgrs/GaoWGDW19, DBLP:journals/tgrs/GengMZW19, DBLP:journals/lgrs/GaoDLX16, DBLP:journals/tnn/GongZLMJ16, DBLP:journals/tgrs/LiPCJZS19, DBLP:journals/staeors/GaoGDW19, DBLP:journals/lgrs/QuGDDL22, DBLP:journals/tgrs/VinholiPSMP22, DBLP:journals/staeors/WangGDZD22}} & \cite{DBLP:journals/lgrs/MengGDDL22}\\
    \hline
    \textbf{Multi-spectral based} & \makecell[l]{\cite{DBLP:journals/tgrs/HeZZ20} \cite{DBLP:journals/tip/TouatiMD20} \cite{DBLP:journals/lgrs/WangCBLC15} \cite{DBLP:journals/lgrs/HaoZJS20} \cite{DBLP:journals/tgrs/VongsyEM15} \cite{DBLP:journals/tgrs/WangAS15a} \\ \cite{DBLP:journals/lgrs/DingHXZP15} \cite{DBLP:journals/tip/ZanettiBB15}  \cite{DBLP:journals/lgrs/AleksandrowiczW16} \cite{DBLP:journals/tgrs/HedjamKMNC16} \cite{DBLP:journals/tgrs/DuRWZ19} \cite{DBLP:journals/tgrs/Padron-HidalgoL19} \\ \cite{DBLP:journals/tgrs/LvLZBLZ19} \cite{DBLP:journals/tgrs/LiLFD16} \cite{DBLP:journals/staeors/ZhouCLS16} \cite{DBLP:journals/staeors/TanJPWXD16}  \cite{DBLP:journals/tip/KrylovMSZ16} \cite{DBLP:journals/lgrs/WuD17} \\ \cite{DBLP:journals/staeors/0012LNZL17} \cite{DBLP:journals/lgrs/LiSZH17} \cite{DBLP:journals/lgrs/WuLFMS18}  \cite{DBLP:journals/lgrs/GuptaPA18} \cite{DBLP:journals/staeors/ZhangLC18} \cite{DBLP:journals/lgrs/ZhangPH18} \\ \cite{DBLP:journals/tgrs/ZanettiB18} \cite{DBLP:journals/tgrs/ZhangLL18} \cite{DBLP:journals/tgrs/LiuGT19} \cite{DBLP:journals/staeors/GongYZNL19}  \cite{DBLP:journals/staeors/FanLH19} \cite{DBLP:journals/tgrs/YangLWYE19} \\ \cite{DBLP:journals/lgrs/CorreaBB19} \cite{DBLP:journals/lgrs/KhuranaS20}  \cite{DBLP:journals/staeors/WangDCLZL20} \cite{DBLP:journals/tgrs/LvLB20} \cite{DBLP:journals/lgrs/WuLNYZ20} \cite{DBLP:journals/corr/abs-2302-05114} \\ \cite{DBLP:journals/lgrs/ZhangLZSZ22} \cite{DBLP:journals/staeors/XiaoWCSQL23} \cite{DBLP:journals/staeors/LiSZGHY22} \cite{DBLP:journals/tgrs/TianZMZ22}  \cite{DBLP:journals/tgrs/Padron-HidalgoL22} \cite{DBLP:journals/lgrs/ShaoYLDR22} \\ \cite{DBLP:journals/lgrs/LvWLKB22} \cite{DBLP:journals/lgrs/FangDWLT22} \cite{DBLP:journals/lgrs/GuoZZZ22} \cite{DBLP:journals/tgrs/MouHSBBZ22} \cite{DBLP:journals/staeors/XueLJWCN21} \cite{DBLP:journals/staeors/ZhouSCZSQ21} \\ \cite{DBLP:journals/tgrs/GuoZ021} \cite{DBLP:journals/tgrs/NegriFCADSA21}\cite{DBLP:journals/sensors/HouWL16}} & \makecell[l]{\cite{DBLP:journals/lgrs/ZhongLZZ15} \cite{DBLP:journals/lgrs/ZhangYGYSYZ22} \cite{DBLP:journals/lgrs/LiHLS22} \cite{DBLP:journals/lgrs/LinLFG20} \cite{DBLP:journals/tgrs/HouLWW20} \cite{DBLP:journals/tgrs/ZhaoMCBE20} \\ \cite{DBLP:journals/lgrs/JiangGZF20} \cite{DBLP:journals/staeors/KalinichevaIST20} \cite{DBLP:journals/lgrs/MesquitaSMCN20} \cite{DBLP:journals/tgrs/ZhanGJZ20} \cite{DBLP:journals/tgrs/ZhangS20} \cite{DBLP:journals/lgrs/ZhangGZSS16} \\ \cite{DBLP:journals/tgrs/MouBZ19} \cite{DBLP:journals/tgrs/GongZZM17} \cite{DBLP:journals/lgrs/HouWL17} \cite{DBLP:journals/lgrs/ZhanFYSWQ17} \cite{9721892} \cite{DBLP:journals/tgrs/KhanHPB17} \cite{DBLP:journals/staeors/KernerWBGBA19} \\ \cite{DBLP:journals/lgrs/ZhangXCYS19} \cite{DBLP:journals/tgrs/YangJLHY19} \cite{DBLP:journals/tgrs/ChenWDZW20} \cite{DBLP:journals/staeors/HedjamAM20} \cite{DBLP:journals/staeors/LiuJZZ20} \cite{DBLP:journals/lgrs/BaoFFH20} \\  \cite{DBLP:journals/corr/abs-2212-01287} \cite{DBLP:journals/corr/abs-2206-11892} \cite{DBLP:journals/tgrs/BergamascoSBB22} \cite{DBLP:journals/tgrs/ShiWQLJ22} \cite{DBLP:journals/lgrs/ShiZTLL22} \cite{DBLP:journals/corr/abs-2108-07955} \\ \cite{DBLP:conf/cvpr/NohJSPC22} \cite{DBLP:journals/tgrs/ChenLCS22} \cite{DBLP:journals/corr/abs-2211-11478} \cite{DBLP:journals/tgrs/FangGWLLD23} \cite{10023508} \cite{DBLP:journals/tcyb/WuCDZ22} \\ \cite{9721897} \cite{DBLP:journals/tgrs/ZhouFHL22} \cite{9978928} \cite{DBLP:journals/corr/abs-2202-09745} \cite{DBLP:journals/lgrs/LiYZM22} \cite{DBLP:journals/staeors/ShiLZWHZSLLZ22} \\ \cite{DBLP:journals/lgrs/SunZHWX22} \cite{DBLP:journals/staeors/HeCLC22} \cite{DBLP:journals/lgrs/JianCC22} \cite{DBLP:journals/lgrs/Radoi22} \cite{DBLP:journals/tgrs/ChenB22b}  \cite{ DBLP:journals/lgrs/JiangXWT22} \\ \cite{DBLP:journals/lgrs/RazaHF22} \cite{DBLP:journals/staeors/DengCYYMCZ22} \cite{DBLP:journals/tgrs/BaiFLL22} \cite{DBLP:journals/tgrs/YangXLDYPZ22} \cite{DBLP:journals/tgrs/YuanMXZ22} \cite{DBLP:journals/tgrs/TangZMLZZJ22} \\ \cite{DBLP:journals/lgrs/SunMWL22} \cite{DBLP:journals/lgrs/HanLZ22} \cite{DBLP:journals/lgrs/DuZDLCZC22} \cite{DBLP:journals/tgrs/RenWGZC21} \cite{DBLP:journals/staeors/ChenLYZDP22} \cite{DBLP:journals/tgrs/XiaTZL22} \\ \cite{DBLP:journals/corr/abs-2302-10420} \cite{DBLP:journals/corr/abs-2302-05109} \cite{DBLP:journals/lgrs/LiuPZZY21}  \cite{DBLP:journals/staeors/TangWZ21} \cite{DBLP:journals/tnn/ZhangLYZ23} \cite{DBLP:journals/lgrs/SahaCBB21} \\ \cite{DBLP:journals/staeors/LuoLWHWJX21} \cite{DBLP:journals/tgrs/YangJHLY21} \cite{DBLP:journals/lgrs/SahaMZBB21} \cite{DBLP:journals/tgrs/PengBZGDH21} \cite{DBLP:journals/tgrs/DingGLMZB22} \cite{DBLP:journals/tgrs/LiuGLZZJZ22} \cite{DBLP:conf/igarss/AlvarezRD20}} & \makecell[l]{\cite{DBLP:journals/lgrs/XiangTLY22} \cite{DBLP:journals/tgrs/ShiLLLWZ22} \cite{DBLP:journals/lgrs/PeiZ22} \cite{DBLP:journals/staeors/ZhaoZGLYXL22} \\ \cite{DBLP:journals/tgrs/LvWCBLS22} \cite{DBLP:journals/tcsv/ZhouWZYCM22} \cite{DBLP:journals/corr/abs-2212-04869} \cite{DBLP:journals/corr/abs-2212-05245} \\ \cite{DBLP:conf/igarss/HafnerBN22} \cite{DBLP:journals/corr/abs-2207-09240} \cite{DBLP:journals/staeors/YuanWC22} \cite{DBLP:journals/staeors/SongXWLQC23} \\ \cite{DBLP:journals/tgrs/LiTLZDWZ23} \cite{DBLP:journals/tgrs/LiuYZDL22} \cite{DBLP:journals/tgrs/LiuSMHLZ22} \cite{DBLP:journals/tgrs/LiZDD22} \\ \cite{DBLP:journals/tgrs/HuangSWY22} \cite{DBLP:journals/staeors/SongHL22} \cite{DBLP:journals/tgrs/ChengWH22} \cite{DBLP:journals/tgrs/FengXJLZ22} \\ \cite{DBLP:journals/tgrs/LiTWZ22} \cite{DBLP:journals/tgrs/ChenQS22} \cite{DBLP:journals/tgrs/LeiWNWX0N22} \cite{DBLP:journals/staeors/ChouhanSC22} \\ \cite{DBLP:journals/lgrs/XuOLWT22} \cite{DBLP:journals/lgrs/SongZLSP22} \cite{DBLP:journals/tgrs/ZhangTXYLYXJZ22} \cite{DBLP:journals/corr/abs-2208-08292} \\ \cite{DBLP:journals/staeors/ChenYPCHZLL21} \cite{DBLP:journals/staeors/LiuCDL22} \cite{9828490} \cite{DBLP:journals/tgrs/GuoZZZZ22} \\ \cite{DBLP:journals/staeors/SongDL22} \cite{DBLP:journals/lgrs/ZhaoCGC22} \cite{doi:10.1080/01431161.2021.1941390}} \\
    \hline
    \textbf{Hyper-spectral based} & \makecell[l]{\cite{DBLP:journals/staeors/HuWZD21} \cite{DBLP:journals/tgrs/MeolaEMA12} \cite{DBLP:journals/tgrs/EismannMH08} \cite{8898697} \cite{DBLP:journals/ijon/WuZD15} \cite{DBLP:journals/tgrs/MarinelliBB19} \\ \cite{DBLP:journals/lgrs/ErturkP15} \cite{DBLP:journals/tgrs/LiuBBD15} \cite{DBLP:journals/staeors/ErturkIP16} \cite{DBLP:journals/staeors/JafarzadehH19} \cite{DBLP:journals/tgrs/ChangKG22} \cite{DBLP:journals/staeors/LiuHNG22} \\ \cite{DBLP:journals/ijon/YuanLL15}} & \makecell[l]{\cite{DBLP:journals/staeors/TongPLLLXX20} \cite{DBLP:journals/tgrs/WangWWB22} \cite{DBLP:journals/staeors/GeTBZXS22} \cite{DBLP:journals/tgrs/WangWWWB22} \cite{DBLP:journals/staeors/ZhanSSJWYW21} \cite{DBLP:journals/staeors/LiGDLHWFHTLM21} \\ \cite{DBLP:journals/tgrs/OuLTZX22} \cite{DBLP:journals/lgrs/ZhaoCF22} \cite{DBLP:journals/tgrs/ShiZZZX22} \cite{Wang2019GETNETAG} \cite{DBLP:journals/jvcir/HuangYF19}} & \makecell[l]{ \cite{DBLP:journals/lgrs/DingLZ22} \cite{DBLP:journals/remotesensing/WangJLXL21} \cite{DBLP:journals/tgrs/GongJQLZLZZ22} \\ \cite{DBLP:journals/tgrs/QuHDLX22} \cite{DBLP:journals/tgrs/HuWZ22} \cite{DBLP:journals/tgrs/LuoZLGGR23} \cite{DBLP:conf/igarss/Hu0022}} \\
    \hline
    \textbf{Heterogeneous based} & \makecell[l]{\cite{DBLP:journals/staeors/ZhouLSWL21} \cite{DBLP:journals/lgrs/LiuMDP14} \cite{DBLP:conf/igarss/MoserALS20} \cite{DBLP:conf/igarss/HanTC22} \cite{DBLP:journals/tip/LiuLMHP18} \cite{DBLP:journals/tgrs/SunLGKL22} \\ \cite{DBLP:journals/tip/SunLGK21} \cite{DBLP:journals/lgrs/ZhanGJL18} \cite{DBLP:journals/staeors/ChenHL22} \cite{DBLP:journals/tgrs/SunLLTK21} \cite{DBLP:journals/tgrs/SunLGLK22} \cite{DBLP:journals/tgrs/LiuZPN22} \\ \cite{DBLP:journals/tgrs/SunLLTK22} \cite{DBLP:journals/tip/PrendesC0GT15} \cite{DBLP:journals/tgrs/WanXY19} \cite{DBLP:journals/staeors/TouatiMD19} \cite{DBLP:journals/lgrs/LeiSK22} \cite{DBLP:journals/staeors/ChirakkalBMBB21} \\ \cite{DBLP:journals/lgrs/ZhengGLCL22} \cite{DBLP:journals/tgrs/SierraQABFC22}} & \makecell[l]{\cite{DBLP:conf/igarss/TomenottiLHMA20} \cite{DBLP:conf/icpr/Yang0CF18} \cite{DBLP:journals/lgrs/JiaZLZW22} \cite{DBLP:journals/staeors/JiangLLZH20} \cite{DBLP:journals/tgrs/ZhaoWGL17} \cite{DBLP:journals/tnn/WuLYQMG22} \\ \cite{DBLP:journals/tgrs/LuppinoKBMSJA22}  \cite{DBLP:journals/staeors/LiGZW21} \cite{DBLP:journals/tnn/LiuGQZ18} \cite{DBLP:journals/lgrs/NiuGZY19} \cite{DBLP:journals/tgrs/JiangLZH22} \cite{DBLP:journals/staeors/TouatiMD20a} \\ \cite{DBLP:journals/lgrs/LvHGBZS22} \cite{DBLP:journals/tgrs/SahaEZ22} \cite{DBLP:journals/tgrs/HuLX22} \cite{DBLP:journals/tnn/YangJLHYJ22}\cite{DBLP:journals/aeog/WuLQNZFS21}} & \cite{DBLP:journals/tgrs/WangL22b} \\
    \hline
    \textbf{3D point cloud based} & \makecell[l]{\cite{DBLP:journals/staeors/XiaoXEV16} \cite{DBLP:journals/tgrs/MarinelliPB18} \cite{doi:10.1080/17538947.2019.1585975} \cite{8272508} \\ \cite{isprs-annals-IV-2-W7-9-2019} \cite{isprs-annals-V-2-2020-687-2020}  \cite{isprs-annals-IV-2-W5-357-2019}} & \cite{DEGELIS2023274} & \cite{MARSOCCI2023325} \\
    \hline\hline
  \end{tabular}
  \label{tab:data_learning_strategy_backup}
\end{table*}


Sure, I'd be happy to introduce you to the three main types of machine learning in AI techniques: supervised learning, semi-supervised learning, and unsupervised learning.

Supervised learning: Supervised learning is a type of machine learning in which the algorithm is trained using labeled data. Labeled data refers to data where the correct output is already known, and the algorithm uses this labeled data to learn how to make accurate predictions on new, unseen data. The algorithm is given input data and corresponding output data (labels), and it learns to predict the correct output for new input data based on the patterns it has learned from the labeled data. Examples of supervised learning include image classification, speech recognition, and sentiment analysis.

Semi-supervised learning: Semi-supervised learning is a type of machine learning in which the algorithm is trained using both labeled and unlabeled data. Unlabeled data refers to data where the correct output is not known, and the algorithm must learn to identify patterns in the data without any guidance. Semi-supervised learning is useful when labeled data is scarce or expensive to obtain. The algorithm uses the labeled data to learn how to make accurate predictions on new, unseen data, and it uses the unlabeled data to identify patterns that can help it make better predictions. Examples of semi-supervised learning include object recognition and speech recognition.

Unsupervised learning: Unsupervised learning is a type of machine learning in which the algorithm is trained using only unlabeled data. The algorithm is tasked with finding patterns and structure in the data without any guidance or labels. The algorithm identifies relationships and groupings in the data and uses these relationships to learn about the underlying structure of the data. Unsupervised learning is useful for discovering hidden patterns and relationships in data, and it is often used in applications such as clustering, anomaly detection, and dimensionality reduction.

These are the three main types of machine learning in AI techniques. Each type has its strengths and weaknesses, and the type of learning used will depend on the specific problem being solved and the available data.

\par \textbf{Supervised learning:}
Advantages:
Supervised learning is easy to understand and implement as the labeled data is readily available.
The performance of the model can be easily measured using metrics such as accuracy, precision, and recall.
Supervised learning can be used to solve a wide range of problems such as classification, regression, and ranking.
Disadvantages:

Supervised learning requires a large amount of labeled data, which can be expensive and time-consuming to obtain.
The performance of the model is highly dependent on the quality of the labeled data. If the labeled data is biased or inaccurate, the model's performance will suffer.
Supervised learning models can struggle with data that is different from the training data, leading to overfitting or underfitting.
\par \textbf{Semi-supervised learning:}
Advantages:
Semi-supervised learning can be used when labeled data is scarce or expensive to obtain, allowing for more efficient use of resources.
The use of unlabeled data can help improve the accuracy of the model by allowing it to generalize better to new data.
Semi-supervised learning can be used to solve a wide range of problems, including classification and regression.
Disadvantages:
Semi-supervised learning can be difficult to implement as the algorithm needs to be able to effectively use both labeled and unlabeled data.
The performance of the model can be highly dependent on the quality of the unlabeled data, which can be difficult to assess.
The use of unlabeled data can introduce noise into the model, leading to decreased performance.
\par \textbf{Unsupervised learning:}
Advantages:
Unsupervised learning can be used to find patterns and relationships in data without any prior knowledge or assumptions.
Unsupervised learning can be used to solve a wide range of problems, including clustering, anomaly detection, and dimensionality reduction.
Unsupervised learning can be used when labeled data is not available, making it more flexible than supervised learning.
Disadvantages:

Unsupervised learning can be difficult to interpret, as the results are not based on any pre-defined labels or targets.
The performance of the model can be highly dependent on the quality of the data and the choice of algorithm, making it more challenging to optimize than supervised learning.
Unsupervised learning can suffer from the "curse of dimensionality," where the performance of the model decreases as the number of dimensions (features) increases.
\par These are the advantages and disadvantages of the three main types of machine learning in AI techniques. Choosing the appropriate type of learning will depend on the specific problem being solved, the available data, and the resources and constraints of the project.


 \section{Benchmark Performance} % 2-3 pages
  \label{benchmark}
  \gl{add the benchmark performance by Yunmeng}
  \subsubsection{SAR based Benchmarks}  
\begin{table*}[!ht]
  \centering
  \caption{Representative methods on popular datasets.}
  \scalebox{1.0}{
  \begin{tabular}
  {p{0.15\textwidth}|p{0.10\textwidth} |p{0.08\textwidth}|p{0.06\textwidth} |p{0.06\textwidth}|p{0.06\textwidth}
  |p{0.06\textwidth}}
    %\toprule %{c|l|m{7cm}}
    \hline\hline

  \rowcolor{gray!60!}  \multicolumn{7}{c} {\textbf{SAR based Methods}}  \\
    \hline\hline
  \rowcolor{gray!30!}  \makecell[c]{\textbf{Method}} & \makecell[c]{\textbf{Source}} & \makecell[c]{\textbf{Backbone}} & \makecell[c]{\textbf{FP}} & \makecell[c]{\textbf{FN}} & \makecell[c]{\textbf{OA}} & \makecell[c]{\textbf{KC}}\\  
    \hline\hline
  \rowcolor{gray!15!}   \multicolumn{7}{c}{\textbf{Yellow River Dataset}} \\
    \hline\hline
    
    \makecell[c]{PCAKM~\cite{5196726}} & \makecell[c]{GRSL 2009} & \makecell[c]{--} & \makecell[c]{955}  & \makecell[c]{1515} & \makecell[c]{97.57} & \makecell[c]{90.73} \\
    \hline
    \makecell[c]{RFLICM~\cite{6035777}} & \makecell[c]{TIP 2012} & \makecell[c]{--} & \makecell[c]{862} & \makecell[c]{1300} & \makecell[c]{98.33} & \makecell[c]{74.97}  \\
    \hline
    \makecell[c]{GaborPCANet~\cite{DBLP:journals/lgrs/GaoDLX16}} & \makecell[c]{GRSL 2016} & \makecell[c]{PCANet} & \makecell[c]{1043} & \makecell[c]{1009} & \makecell[c]{96.87} & \makecell[c]{81.21}  \\
    \hline
    \makecell[c]{CWNNs~\cite{8641484}} & \makecell[c]{GRSL 2019} & \makecell[c]{--} & \makecell[c]{837} & \makecell[c]{1690} & \makecell[c]{96.60} & \makecell[c]{88.23}  \\
    \hline
    \makecell[c]{DCNet~\cite{DBLP:journals/staeors/GaoGDW19}} & \makecell[c]{J-STARS 2019} & \makecell[c]{--} & \makecell[c]{790} & \makecell[c]{2137} & \makecell[c]{96.06} & \makecell[c]{86.16}  \\
    \hline
    \makecell[c]{MSAPNet~\cite{DBLP:conf/igarss/WangDCLZJ20}} & \makecell[c]{IGARSS 2020} & \makecell[c]{--} & \makecell[c]{817} & \makecell[c]{2157} & \makecell[c]{96.00} & \makecell[c]{85.94}  \\
    \hline
    \makecell[c]{DDNet~\cite{DBLP:journals/lgrs/QuGDDL22}} & \makecell[c]{GRSL 2022} & \makecell[c]{MRC} & \makecell[c]{\textbf{641}} & \makecell[c]{1027} & \makecell[c]{98.36} & \makecell[c]{\textbf{93.77}}  \\
    \hline
    \makecell[c]{SFCNet~\cite{DBLP:journals/tgrs/ZhangJLYSL22}} & \makecell[c]{TGRS 2022} & \makecell[c]{MO-SFL} & \makecell[c]{720} & \makecell[c]{\textbf{704}} & \makecell[c]{\textbf{98.40}} & \makecell[c]{85.62}  \\
    \hline
    \makecell[c]{SSN~\cite{10016644}} & \makecell[c]{GRSL 2023} & \makecell[c]{--} & \makecell[c]{1292} & \makecell[c]{793} & \makecell[c]{97.19} & \makecell[c]{90.66}  \\
    \hline\hline

 
  \rowcolor{gray!15!}   \multicolumn{7}{c}{\textbf{Bern Dataset}} \\
    \hline\hline
    \makecell[c]{PCAKM~\cite{5196726}} & \makecell[c]{GRSL 2009} & \makecell[c]{--} & \makecell[c]{244} & \makecell[c]{\textbf{117}} & \makecell[c]{99.60} & \makecell[c]{84.78}\\
    \hline
    \makecell[c]{GaborPCANet~\cite{DBLP:journals/lgrs/GaoDLX16}} & \makecell[c]{GRSL 2016} & \makecell[c]{PCANet} & \makecell[c]{\textbf{36}} & \makecell[c]{434} & \makecell[c]{99.48} & \makecell[c]{75.23}  \\
    \hline
    \makecell[c]{CWNNs~\cite{8641484}} & \makecell[c]{GRSL 2019} & \makecell[c]{--} & \makecell[c]{81} & \makecell[c]{226} & \makecell[c]{99.66} & \makecell[c]{85.56}  \\
    \hline
    \makecell[c]{ESMOFCM~\cite{9134375}} & \makecell[c]{GRSL 2021} & \makecell[c]{--} & \makecell[c]{95} & \makecell[c]{196} & \makecell[c]{\textbf{99.68}} & \makecell[c]{86.70}  \\
    \hline
    \makecell[c]{BIFLICM/D~\cite{DBLP:journals/lgrs/FangX22}} & \makecell[c]{GRSL 2022} & \makecell[c]{--} & \makecell[c]{103} & \makecell[c]{718} & \makecell[c]{99.08} & \makecell[c]{91.24}  \\
    \hline
    \makecell[c]{ShearNet~\cite{9982693}} & \makecell[c]{TGRS 2022} & \makecell[c]{} & \makecell[c]{163} & \makecell[c]{126} & \makecell[c]{\textbf{99.68}} & \makecell[c]{\textbf{87.41}}  \\
    \hline\hline
  \end{tabular}}
  \label{tab:data_learning_strategy}
\end{table*}

  \subsubsection{Multi-spectral based Benchmarks}
\begin{table*}[!ht]
  \centering
  \caption{Representative methods on popular datasets.}
  \scalebox{1.0}{
  \begin{tabular}
  {p{0.15\textwidth}|p{0.14\textwidth} |p{0.08\textwidth}|p{0.08\textwidth} |p{0.06\textwidth}|p{0.06\textwidth}
  |p{0.06\textwidth}|p{0.06\textwidth}}
    %\toprule %{c|l|m{7cm}}
    \hline\hline

  \rowcolor{gray!60!}  \multicolumn{8}{c} {\textbf{Multispctral based Methods}}  \\
    \hline\hline
  \rowcolor{gray!30!}  \makecell[c]{\textbf{Method}} & \makecell[c]{\textbf{Source}} & \makecell[c]{\textbf{Backbone}} & \makecell[c]{\textbf{Precision}} & \makecell[c]{\textbf{Recall}} & \makecell[c]{\textbf{F1 score}} & \makecell[c]{\textbf{OA}} & \makecell[c]{\textbf{IoU}}\\  
    \hline\hline
  \rowcolor{gray!15!}   \multicolumn{8}{c}{\textbf{LEVIR\_CD Dataset}} \\
    \hline\hline  
    \makecell[c]{FC-EF~\cite{8451652}} & \makecell[c]{ICIP 2018} & \makecell[c]{U-Net} & \makecell[c]{90.64}  & \makecell[c]{78.84} & \makecell[c]{84.33} & \makecell[c]{98.39} & \makecell[c]{71.53}\\
    \hline
    \makecell[c]{STANet~\cite{Chen2020}} & \makecell[c]{Remote Sensing \\ 2020} & \makecell[c]{ResNet} & \makecell[c]{83.81} & \makecell[c]{\textbf{91.00}} & \makecell[c]{87.26} & \makecell[c]{ 98.66} & \makecell[c]{77.40} \\
    \hline
    \makecell[c]{ChangeStar~\cite{9709950}} & \makecell[c]{ICCV 2021} & \makecell[c]{ResNet-50} & \makecell[c]{} & \makecell[c]{\textbf{}} & \makecell[c]{90.82} & \makecell[c]{} & \makecell[c]{\textbf{83.19}} \\
    \hline
    \makecell[c]{ChangeFormer~\cite{9883686}} & \makecell[c]{IGARSS 2022} & \makecell[c]{Transformer} & \makecell[c]{92.05} & \makecell[c]{88.80} & \makecell[c]{90.40} & \makecell[c]{\textbf{99.04}} & \makecell[c]{82.48}  \\
    \hline
    \makecell[c]{BIT~\cite{9491802}} & \makecell[c]{TGRS 2022} & \makecell[c]{ResNet-18} & \makecell[c]{89.24} & \makecell[c]{89.37} & \makecell[c]{89.31} & \makecell[c]{98.92} & \makecell[c]{80.68} \\
    \hline
   \makecell[c]{SNUNet~\cite{9355573}} & \makecell[c]{GRSL 2022} & \makecell[c]{} & \makecell[c]{89.18} & \makecell[c]{87.17} & \makecell[c]{88.16} & \makecell[c]{98.82} & \makecell[c]{78.83} \\
    \hline
    \makecell[c]{P2V-CD~\cite{9975266}} & \makecell[c]{TIP 2023} & \makecell[c]{} & \makecell[c]{\textbf{93.32}} & \makecell[c]{90.60} & \makecell[c]{\textbf{91.94}} & \makecell[c]{} & \makecell[c]{} \\
    \hline\hline
    
  \rowcolor{gray!15!}   \multicolumn{8}{c}{\textbf{CDD Dataset}} \\
    \hline\hline
    \makecell[c]{FC-EF~\cite{8451652}} & \makecell[c]{ICIP 2018} & \makecell[c]{U-Net} & \makecell[c]{83.45} & \makecell[c]{\textbf{98.47}} & \makecell[c]{90.34} & \makecell[c]{97.58} & \makecell[c]{}  \\
    \hline
    \makecell[c]{STANet~\cite{Chen2020}} & \makecell[c]{Remote Sensing \\ 2020} & \makecell[c]{ResNet} & \makecell[c]{95.17} & \makecell[c]{92.88} & \makecell[c]{94.01} & \makecell[c]{} & \makecell[c]{} \\
    \hline
    \makecell[c]{ESCNet~\cite{9474911}} & \makecell[c]{TNNLS 2021} & \makecell[c]{} & \makecell[c]{90.04} & \makecell[c]{97.26} & \makecell[c]{93.51} & \makecell[c]{98.45} & \makecell[c]{} \\
    \hline
    \makecell[c]{ChangeFormer~\cite{9883686}} & \makecell[c]{IGARSS 2022} & \makecell[c]{Transformer} & \makecell[c]{94.50} & \makecell[c]{93.51} & \makecell[c]{94.23} & \makecell[c]{} & \makecell[c]{} \\
    \hline
    \makecell[c]{BIT~\cite{9491802}} & \makecell[c]{TGRS 2022} & \makecell[c]{ResNet-18} & \makecell[c]{96.07} & \makecell[c]{93.49} & \makecell[c]{94.76} & \makecell[c]{} & \makecell[c]{} \\
    \hline
    \makecell[c]{SNUNet~\cite{9355573}} & \makecell[c]{GRSL 2022} & \makecell[c]{} & \makecell[c]{98.09} & \makecell[c]{97.42} & \makecell[c]{97.75} & \makecell[c]{} & \makecell[c]{} \\
    \hline
    \makecell[c]{DSAMNet~\cite{DBLP:journals/tgrs/ShiLLLWZ22}} & \makecell[c]{TGRS 2022} & \makecell[c]{ResNet-18} & \makecell[c]{94.54} & \makecell[c]{92.77} & \makecell[c]{93.69} & \makecell[c]{} & \makecell[c]{} \\
    \hline
    \makecell[c]{P2V-CD~\cite{9975266}} & \makecell[c]{TIP 2023} & \makecell[c]{} & \makecell[c]{\textbf{98.57}} & \makecell[c]{98.26} & \makecell[c]{\textbf{98.42}} & \makecell[c]{} & \makecell[c]{} \\
    \hline\hline
  
  \rowcolor{gray!15!}   \multicolumn{8}{c}{\textbf{WHU Building Dataset}} \\
    \hline\hline
    \makecell[c]{FC-EF~\cite{8451652}} & \makecell[c]{ICIP 2018} & \makecell[c]{U-Net} & \makecell[c]{71.63}  & \makecell[c]{67.25} & \makecell[c]{69.37} & \makecell[c]{97.61} & \makecell[c]{53.11}\\
    \hline
    \makecell[c]{STANet~\cite{Chen2020}} & \makecell[c]{Remote Sensing \\ 2020} & \makecell[c]{ResNet} & \makecell[c]{79.37} & \makecell[c]{85.50} & \makecell[c]{82.32} & \makecell[c]{98.52} & \makecell[c]{69.95} \\
    \hline
    \makecell[c]{DASNet~\cite{DBLP:journals/staeors/ChenYPCHZLL21}} & \makecell[c]{JSTARS 2020} & \makecell[c]{ResNet-50} & \makecell[c]{90.00} & \makecell[c]{\textbf{90.50}} & \makecell[c]{91.00} & \makecell[c]{99.10} & \makecell[c]{} \\
    \hline
    \makecell[c]{ChangeFormer~\cite{9883686}} & \makecell[c]{IGARSS 2022} & \makecell[c]{Transformer} & \makecell[c]{91.83} & \makecell[c]{88.02} & \makecell[c]{89.88} & \makecell[c]{\textbf{99.12}} & \makecell[c]{\textbf{81.63}}  \\
    \hline
    \makecell[c]{BIT~\cite{9491802}} & \makecell[c]{TGRS 2022} & \makecell[c]{ResNet-18} & \makecell[c]{86.64} & \makecell[c]{81.48} & \makecell[c]{83.98} & \makecell[c]{98.75} & \makecell[c]{72.39} \\
    \hline
   \makecell[c]{SNUNet~\cite{9355573}} & \makecell[c]{GRSL 2022} & \makecell[c]{} & \makecell[c]{89.90} & \makecell[c]{86.82} & \makecell[c]{88.33} & \makecell[c]{} & \makecell[c]{} \\
    \hline
    \makecell[c]{P2V-CD~\cite{9975266}} & \makecell[c]{TIP 2023} & \makecell[c]{} & \makecell[c]{\textbf{95.48}} & \makecell[c]{89.47} & \makecell[c]{\textbf{92.38}} & \makecell[c]{} & \makecell[c]{} \\
    \hline\hline

  \rowcolor{gray!15!}   \multicolumn{8}{c}{\textbf{SECOND Dataset}} \\
    \hline\hline  
  \rowcolor{gray!30!}  \makecell[c]{\textbf{Method}} & \makecell[c]{\textbf{Source}} & \makecell[c]{\textbf{Backbone}} & \makecell[c]{\textbf{OA}} & \makecell[c]{\textbf{mIoU}} & \makecell[c]{\textbf{Sek}} & \makecell[c]{$\boldsymbol{F_{scd}}$}  \\  
    \hline\hline
    \makecell[c]{HRSCD~\cite{Daudt2018MultitaskLF}} & \makecell[c]{CVIU 2019} & \makecell[c]{} & \makecell[c]{86.62}  & \makecell[c]{71.15} & \makecell[c]{18.80} & \makecell[c]{58.21} 
  \\
    \hline
    \makecell[c]{SCanNet~\cite{Ding2022JointSM}} & \makecell[c]{arXiv} & \makecell[c]{} & \makecell[c]{87.76} & \makecell[c]{\textbf{73.42}} & \makecell[c]{23.94} & \makecell[c]{63.66}  \\
    \hline
    \makecell[c]{ASN~\cite{DBLP:journals/tgrs/YangXLDYPZ22}} & \makecell[c]{TGRS 2021} & \makecell[c]{} & \makecell[c]{} & \makecell[c]{69.50} & \makecell[c]{16.30} & \makecell[c]{} \\
    \hline
    \makecell[c]{SSCD~\cite{DBLP:journals/tgrs/DingGLMZB22}} & \makecell[c]{TGRS 2022} & \makecell[c]{} & \makecell[c]{87.19} & \makecell[c]{72.60} & \makecell[c]{21.86} & \makecell[c]{61.22}   \\
    \hline
    \makecell[c]{SSESN~\cite{DBLP:journals/staeors/ZhaoZGLYXL22}} & \makecell[c]{J-STARS 2022} & \makecell[c]{} & \makecell[c]{89.00} & \makecell[c]{70.80} & \makecell[c]{} & \makecell[c]{}  \\
    \hline\hline
   \end{tabular}}
  \label{tab:data_learning_strategy}
\end{table*}  

  \subsubsection{Hyper-spectral based Benchmarks}
\begin{table*}[!ht]
  \centering
  \caption{Representative methods on popular datasets.}
  \scalebox{1.0}{
  \begin{tabular}
  {p{0.15\textwidth}|p{0.10\textwidth} |p{0.08\textwidth}|p{0.08\textwidth} |p{0.06\textwidth}|p{0.06\textwidth}
  |p{0.06\textwidth}|p{0.06\textwidth}}
    %\toprule %{c|l|m{7cm}}
    \hline\hline

  \rowcolor{gray!60!}  \multicolumn{8}{c} {\textbf{Hyperspctral based Methods}}  \\
    \hline\hline
  \rowcolor{gray!30!}  \makecell[c]{\textbf{Method}} & \makecell[c]{\textbf{Source}} & \makecell[c]{\textbf{Backbone}} & \makecell[c]{\textbf{Precision}} & \makecell[c]{\textbf{Recall}} & \makecell[c]{\textbf{F1 score}} & \makecell[c]{\textbf{OA}} & \makecell[c]{\textbf{KC}}\\  
    \hline\hline
  \rowcolor{gray!15!}   \multicolumn{8}{c}{\textbf{River Dataset}} \\
    \hline\hline  
    \makecell[c]{CVA~\cite{1980Change}} & \makecell[c]{1980} & \makecell[c]{} & \makecell[c]{61.56}  & \makecell[c]{89.16} & \makecell[c]{72.84} & \makecell[c]{94.22} & \makecell[c]{69.72}\\
    \hline
    \makecell[c]{SVM~\cite{Nemmour2006MultipleSV}} & \makecell[c]{ISPRS 2006} & \makecell[c]{} & \makecell[c]{90.17} & \makecell[c]{69.79} & \makecell[c]{78.68} & \makecell[c]{96.71} & \makecell[c]{76.93} \\
    \hline
    \makecell[c]{PCA-CVA~\cite{DBLP:journals/lgrs/ZhangGZSS16}} & \makecell[c]{GRSL 2016} & \makecell[c]{} & \makecell[c]{} & \makecell[c]{} & \makecell[c]{} & \makecell[c]{95.16} & \makecell[c]{74.77} \\
    \hline
    \makecell[c]{GETNET~\cite{Wang2019GETNETAG}} & \makecell[c]{TGRS 2018} & \makecell[c]{CNN} & \makecell[c]{85.64} & \makecell[c]{78.98} & \makecell[c]{82.18} & \makecell[c]{97.18} & \makecell[c]{80.53}  \\
    \hline
    \makecell[c]{SSA-SiamNet~\cite{9494085}} & \makecell[c]{TGRS 2021} & \makecell[c]{} & \makecell[c]{91.89} & \makecell[c]{74.10} & \makecell[c]{82.04} & \makecell[c]{97.18} & \makecell[c]{80.53} \\
    \hline
   \makecell[c]{MSDFFN~\cite{DBLP:journals/tgrs/LuoZLGGR23}} & \makecell[c]{TGRS 2023} & \makecell[c]{} & \makecell[c]{\textbf{97.79}} & \makecell[c]{\textbf{97.77}} & \makecell[c]{\textbf{97.78}} & \makecell[c]{\textbf{98.71}} & \makecell[c]{\textbf{96.88}} \\
    \hline\hline
    
  \rowcolor{gray!15!}   \multicolumn{8}{c}{\textbf{Hermiston Dataset}} \\
    \hline\hline
\makecell[c]{CVA~\cite{1980Change}} & \makecell[c]{1980} & \makecell[c]{} & \makecell[c]{\textbf{97.61}}  & \makecell[c]{74.63} & \makecell[c]{84.59} & \makecell[c]{93.87} & \makecell[c]{80.85}\\
    \hline
    \makecell[c]{SVM~\cite{Nemmour2006MultipleSV}} & \makecell[c]{ISPRS 2006} & \makecell[c]{} & \makecell[c]{94.17} & \makecell[c]{88.03} & \makecell[c]{91.00} & \makecell[c]{96.08} & \makecell[c]{88.49} \\
    \hline
    \makecell[c]{GETNET~\cite{Wang2019GETNETAG}} & \makecell[c]{TGRS 2018} & \makecell[c]{CNN} & \makecell[c]{92.99} & \makecell[c]{90.16} & \makecell[c]{91.50} & \makecell[c]{89.09} & \makecell[c]{\textbf{96.23}}  \\
    \hline
    \makecell[c]{SSA-SiamNet~\cite{9494085}} & \makecell[c]{TGRS 2021} & \makecell[c]{} & \makecell[c]{93.18} & \makecell[c]{89.17} & \makecell[c]{91.45} & \makecell[c]{96.22} & \makecell[c]{89.02} \\
    \hline
    \makecell[c]{RSCNet~\cite{DBLP:journals/tgrs/WangWWB22}} & \makecell[c]{TGRS 2022} & \makecell[c]{ResNet-50} & \makecell[c]{93.98} & \makecell[c]{91.32} & \makecell[c]{92.63} & \makecell[c]{96.73} & \makecell[c]{90.53} \\
    \hline
   \makecell[c]{MSDFFN~\cite{DBLP:journals/tgrs/LuoZLGGR23}} & \makecell[c]{TGRS 2023} & \makecell[c]{} & \makecell[c]{95.55} & \makecell[c]{\textbf{93.69}} & \makecell[c]{\textbf{94.61}} & \makecell[c]{\textbf{97.59}} & \makecell[c]{93.06} \\
    \hline\hline
  \end{tabular}}
  \label{tab:data_learning_strategy}
\end{table*}   

  \subsubsection{Hetergenous based Benchmarks}
\begin{table*}[!ht]
  \centering
  \caption{Representative methods on popular datasets.}
  \scalebox{1.0}{
  \begin{tabular}
  {p{0.15\textwidth}|p{0.10\textwidth} |p{0.08\textwidth}|p{0.08\textwidth} |p{0.06\textwidth}|p{0.06\textwidth}
  |p{0.06\textwidth}}
    %\toprule %{c|l|m{7cm}}
    \hline\hline

  \rowcolor{gray!60!}  \multicolumn{7}{c} {\textbf{Heterogeneous based Methods}}  \\
    \hline\hline
  \rowcolor{gray!30!}  \makecell[c]{\textbf{Method}} & \makecell[c]{\textbf{Source}} & \makecell[c]{\textbf{Backbone}} & \makecell[c]{\textbf{OA}} & \makecell[c]{\textbf{KC}} & \makecell[c]{\textbf{AUC}} & \makecell[c]{\textbf{F1 score}}  \\  
    \hline\hline
  \rowcolor{gray!15!}   \multicolumn{7}{c}{\textbf{California Dataset}} \\
    \hline\hline  
    \makecell[c]{SCCN~\cite{DBLP:journals/tnn/LiuGQZ18}} & \makecell[c]{TNNLS 2018} & \makecell[c]{} & \makecell[c]{97.60}  & \makecell[c]{87.17} & \makecell[c]{98.78} & \makecell[c]{} 
 \\
    \hline
    \makecell[c]{AM\_HPT~\cite{8798991}} & \makecell[c]{TGRS 2019} & \makecell[c]{} & \makecell[c]{98.12} & \makecell[c]{90.18} & \makecell[c]{99.24} & \makecell[c]{}  \\
    \hline
    \makecell[c]{CAN~\cite{DBLP:journals/lgrs/NiuGZY19}} & \makecell[c]{GRSL 2019} & \makecell[c]{GAN} & \makecell[c]{90.40} & \makecell[c]{36.50} & \makecell[c]{} & \makecell[c]{42.40}  \\
    \hline
    \makecell[c]{ACE-Net~\cite{DBLP:journals/tgrs/LuppinoKBMSJA22}} & \makecell[c]{TGRS 2021} & \makecell[c]{} & \makecell[c]{91.50} & \makecell[c]{41.50} & \makecell[c]{} & \makecell[c]{45.90}  \\
    \hline
    \makecell[c]{CA\_AE~\cite{9773305}} & \makecell[c]{TNNLS 2022} & \makecell[c]{} & \makecell[c]{97.88} & \makecell[c]{88.66} & \makecell[c]{99.18} & \makecell[c]{}  \\
    \hline
   \makecell[c]{DPFL-Net-4~\cite{DBLP:journals/tnn/YangJLHYJ22}} & \makecell[c]{TNNLS 2022} & \makecell[c]{} & \makecell[c]{\textbf{98.89}} & \makecell[c]{\textbf{94.17}} & \makecell[c]{\textbf{99.79}} & \makecell[c]{}  \\
    \hline\hline
  \end{tabular}}
  \label{tab:data_learning_strategy}
\end{table*}

  \subsubsection{Point cloud based Benchmarks}
\begin{table*}[!ht]
  \centering
  \caption{Representative methods on popular datasets.}
  \scalebox{1.0}{
  \begin{tabular}
  {p{0.15\textwidth}|p{0.10\textwidth} |p{0.08\textwidth}|p{0.06\textwidth} |p{0.06\textwidth}}
    %\toprule %{c|l|m{7cm}}
    \hline\hline

  \rowcolor{gray!60!}  \multicolumn{5}{c} {\textbf{Heterogeneous based Methods}}  \\
    \hline\hline
  \rowcolor{gray!30!}  \makecell[c]{\textbf{Method}} & \makecell[c]{\textbf{Source}} & \makecell[c]{\textbf{Backbone}} & \makecell[c]{\textbf{RMSE}} & \makecell[c]{\textbf{cRMSE}}  \\  
    \hline\hline
  \rowcolor{gray!15!}   \multicolumn{5}{c}{\textbf{3DCD Dataset}} \\
    \hline\hline  
    \makecell[c]{IM2HEIGHT~\cite{Mou2018IM2HEIGHTHE}} & \makecell[c]{arXiv} & \makecell[c]{} & \makecell[c]{1.57}  & \makecell[c]{7.59} 
 \\
    \hline
    \makecell[c]{FC-EF~\cite{8451652}} & \makecell[c]{ICIP 2018} & \makecell[c]{} & \makecell[c]{1.41} & \makecell[c]{7.04}  \\
    \hline
    \makecell[c]{ChangeFormer~\cite{9883686}} & \makecell[c]{IGARSS 2022} & \makecell[c]{Transformer} & \makecell[c]{1.31} & \makecell[c]{7.09}   \\
    \hline
    \makecell[c]{SNUNet~\cite{9355573}} & \makecell[c]{GRSL 2022} & \makecell[c]{} & \makecell[c]{1.24} & \makecell[c]{6.47}  \\
    \hline
    \makecell[c]{MTBIT~\cite{MARSOCCI2023325}} & \makecell[c]{ISPRS 2023} & \makecell[c]{} & \makecell[c]{\textbf{1.20}} & \makecell[c]{\textbf{6.46}}  \\
    \hline\hline
  \end{tabular}}
  \label{tab:data_learning_strategy}
\end{table*}
